Longitudinal cardio-respiratory fitness prediction through wearables in free-living environments

Cardiorespiratory fitness is an established predictor of metabolic disease and mortality. Fitness is directly measured as maximal oxygen consumption (VO$_{2}max$), or indirectly assessed using heart rate responses to standard exercise tests. However, such testing is costly and burdensome because it requires specialized equipment such as treadmills and oxygen masks, limiting its utility. Modern wearables capture dynamic real-world data which could improve fitness prediction. In this work, we design algorithms and models that convert raw wearable sensor data into cardiorespiratory fitness estimates. We validate these estimates' ability to capture fitness profiles in free-living conditions using the Fenland Study (N=11,059), along with its longitudinal cohort (N=2,675), and a third external cohort using the UK Biobank Validation Study (N=181) who underwent maximal VO$_{2}max$ testing, the gold standard measurement of fitness. Our results show that the combination of wearables and other biomarkers as inputs to neural networks yields a strong correlation to ground truth in a holdout sample (r = 0.82, 95CI 0.80-0.83), outperforming other approaches and models and detects fitness change over time (e.g., after 7 years). We also show how the model's latent space can be used for fitness-aware patient subtyping paving the way to scalable interventions and personalized trial recruitment. These results demonstrate the value of wearables for fitness estimation that today can be measured only with laboratory tests.

==> ResearchInContext.tex <==
% \noindent
% \fbox{\begin{minipage}[t]{.45\textwidth}
% \raggedright
% This is \\
% some left-aligned \\
% text in a column \\
% for demo purposes
% \end{minipage}}
% \hfill
% \noindent
% \fbox{\begin{minipage}[t]{.45\textwidth}
% \raggedleft
% This is \\
% some different \\
% text, right-aligned \\
% for demo purposes, \\
% and with more lines.
% \end{minipage}}

\subsection*{Evidence before this study}
Large-scale assessment of physical activity and heart rate data could enable training robust models that anticipate and predict fine-grained changes of fitness over time. Current fitness estimation models, however, have limitations.
%is not easily accessible. 
%\cm{what is meant by not easily accessible?}\jh{changed}
We searched the PubMed database %without language or date restrictions 
for publications up to April 27 2022, for studies about VO2max estimation through wearables, using the search criteria "Vo2max AND wearable" and "Vo2max AND machine learning". We should note that the intersection of the three terms "Vo2max AND machine learning AND wearable" yielded only one result. We systematically screened all 34 results (21, 12, 1 from each respective search) by reviewing abstracts, and identified five original research studies which were relevant to the study aims. These studies were either small-scale assessments of VO2max or required data collected from non free-living environments. We discuss these studies in further detail in the respective sections of this paper.

\vspace{0.2cm}
\subsection*{Added value of this study}
In this study, deep learning models were developed for remote and scalable estimation of cardio-respiratory fitness through wearable devices. Our study expands on previous studies by being the first large-scale study integrating a large cohort, a longitudinal validation cohort, and a third gold standard cohort. The deep learning model takes statistical features extracted from the raw sensor timeseries covering movement and heart rate attributes, and returns fine-grained predictions of VO2max, either in the present or the future. We independently validated the models on several holdout test sets (different participants from the set used when training the AI model). Our results show that using passive sensor data from everyday life can improve fitness prediction significantly, opening the door to population-scale assessment of fitness, moving beyond traditional predictors of individuals' health such as weight or BMI.

\vspace{0.2cm}
\subsection*{Implications of all the available evidence}
The performance of our deep learning-based sensor analysis model suggests that it can potentially be used for fitness estimation with similar accuracy to a laboratory-measured test.
In the future, wearables could include additional sensors which could further improve fitness prediction, such as blood pressure, skin conductance, and oximetry. Future prospective studies will help to identify the impact of personalized fitness predictions by suggesting interventions on individuals through lifestyle, nutrition, and exercise recommendations.



%\begin{figure*}[!t]
%\ContinuedFloat
  
 %    \subfigure[]{
%   \includegraphics[width=0.99\textwidth]{figs/progression_user_o1UMpbeXojNe.pdf}    
%   }
%\end{figure*}

==> ablation_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}

\caption{\textbf{Evaluation of predicting fine-grained VO2max with the Fenland I cohort}. Comparison between traditional antrhopometrics, common biomarkers (RHR), and passively collected data over a week (wearable sensors). Best performance in bold. \revised{The units of VO2max are measured in  $ml O_2/min/kg$. Results reported from the testing set.}}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{@{}lllllcl@{}}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Data modality}}                                                                           & \multicolumn{3}{c}{Evaluation Metrics {[}95\% CI{]}}                                                   & \multicolumn{1}{l}{N (train+val / test set)}                                         &  \\ \cmidrule(l){3-7} 
\multicolumn{2}{c}{}                                                                                                         & \multicolumn{1}{c}{R$^{2}$}           & \multicolumn{1}{c}{Corr}         & \multicolumn{1}{c}{RMSE}         & \multirow{13}{*}{\begin{tabular}[c]{@{}c@{}}11059 \\ (8384/2675)\end{tabular}} &  \\ \cmidrule(r){1-5}
\multicolumn{2}{l}{\textbf{Anthropometrics}}                                                                                 &                                  &                                  &                                  &                                                                                &  \\
 & \multirow{1}{*}{Age/Sex/Weight/BMI/Height}                                                                  %              & 0.359 {[}0.328-0.39{]}           & 0.601 {[}0.575-0.626{]}          & 4.050 {[}0.344-0.403{]}          &                                                                                &  \\
% &
& 0.362 {[}0.332-0.391{]}          & 0.604 {[}0.579-0.627{]}          & 4.043 {[}3.924-4.172{]}          &                                                                                &  \\
\multicolumn{2}{l}{\textbf{Resting Heart Rate}}                                                                              &                                  &                                  &                                  &                                                                                &  \\
 & \multirow{1}{*}{RHR (Sensor-derived)}                                                                                              %        & 0.373 {[}0.344-0.408{]}          & 0.613 {[}0.589-0.641{]}          & 4.008 {[}3.888-4.12{]}           &                                                                                &  \\
 %&  
 & 0.374 {[}0.344-0.403{]}          & 0.615 {[}0.589-0.639{]}          & 4.007 {[}3.891-4.117{]}          &                                                                                &  \\
\multicolumn{2}{l}{\textbf{Anthropometrics + RHR}}                                                                           &                                  &                                  &                                  &                                                                                &  \\
 & \multirow{1}{*}{Age/Sex/Weight/BMI/Height/RHR}                                                            %                & 0.610 {[}0.585-0.634{]}          & 0.781 {[}0.765-0.797{]}          & 3.160 {[}3.059-3.266{]}          &                                                                                &  \\
 %& 
 & 0.616 {[}0.588-0.641{]}          & 0.785 {[}0.767-0.802{]}          & 3.138 {[}3.031-3.237{]}          &                                                                                &  \\
\multicolumn{2}{l}{\textbf{Wearable Sensors + RHR + Anthro.}}                                                                &                                  &                                  &                                  &                                                                                &  \\
 & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Acceleration/HR/HRV/MVPA \\  Age/Sex/Weight/BMI/Height/RHR\end{tabular}} 
 %& 0.659 {[}0.628-0.687{]}          & 0.812 {[}0.793-0.83{]}           & 2.956 {[}2.815-3.085{]}          &                                                                                &  \\
 %&
 
 & \textbf{0.671 {[}0.649-0.692{]}} & \textbf{0.822 {[}0.808-0.835{]}} & \textbf{2.903 {[}2.801-3.003{]}} &                                                                                &  \\ \\ \bottomrule
 \label{tab:fenI_results}
\end{tabular}
}

\end{table*}


==> table_study_characteristics.tex <==
\begin{table}
%this goes on top
\caption{\textbf{Characteristics for the study analytical sample: The Fenland I and II studies }} 
\label{tab:cohortcharacteristics}
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
 & \multicolumn{4}{c}{\textbf{Fenland I}} & \multicolumn{4}{c}{\textbf{Fenland II}}\tabularnewline
 \\\cmidrule(lr){2-5}\cmidrule(lr){6-9}
 & \multicolumn{2}{l}{Men (n= 5229)} & \multicolumn{2}{l}{Women (n= 5830)} & \multicolumn{2}{l}{Men (n=1448)} & \multicolumn{2}{l}{Women (n=1593)}\tabularnewline
 \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
 & \textit{N or mean}  & \textit{\% or sd}  & \textit{N or mean}  & \textit{\% or sd}  & \textit{N or mean}  & \textit{\% or sd}  & \textit{N or mean}  & \textit{\% or sd} \tabularnewline
 \midrule
\multicolumn{9}{l}{\textbf{Demographics} }\tabularnewline
\qquad{}Age (years)  & 47.70 & 7.57 & 47.66 & 7.36 & 54.51 & 7.10 & 55.08 & 6.81\tabularnewline
\multicolumn{9}{l}{\textbf{Anthropometrics} }\tabularnewline
\qquad{}Height (m)  & 1.78 & 0.07 & 1.64 & 0.06 & 1.77 & 0.07 & 1.64 & 0.06\tabularnewline
\qquad{}Body mass (kg)  & 85.85 & 13.83 & 70.54 & 13.92 & 85.88 & 14.23 & 70.22 & 14.54\tabularnewline
\qquad{}BMI (kg/m$^{2}$)  & 27.16 & 3.97 & 26.17 & 4.97 & 27.25 & 4.20 & 26.17 & 5.26 \tabularnewline
\qquad{}FMI (kg/m$^{2}$)  & 44.32 & 12.21 & 45.67 & 10.84 & \multicolumn{4}{c}{N.A.}\tabularnewline

\multicolumn{9}{l}{\textbf{Alcohol consumption} }\tabularnewline
\qquad{}$<$1/week & 1328 & 25.4\% & 2262 & 38.8\% & \multicolumn{4}{c}{N.A.}\tabularnewline
\qquad{}1-4/week & 2823 & 54.0\% & 2746 & 35\%  & \multicolumn{4}{c}{N.A.}\tabularnewline
\qquad{}Almost daily & 1009 & 19.3\% & 717 & 12.3\% & \multicolumn{4}{c}{N.A.}\tabularnewline
\multicolumn{9}{l}{\textbf{Smoking status} }\tabularnewline
\qquad{}Never & 2740 & 52.4\% & 3288 & 56.4\% & \multicolumn{4}{c}{N.A.}\tabularnewline
\qquad{}Former & 1757 & 33.6\% & 1883 & 32.3\% & \multicolumn{4}{c}{N.A.}\tabularnewline
\qquad{}Current & 685 & 13.1\% & 618 & 10.6\% & \multicolumn{4}{c}{N.A.}\tabularnewline

\multicolumn{9}{l}{\textbf{Physical activity} }\tabularnewline
\qquad{}MVPA (min/day)  & 104.03 & 72.18 & 73.30 & 57.33 &  &  &  & \tabularnewline
\qquad{}VPA (min/day)  & 12.52 & 18.15 & 6.28 & 11.04 &  &  &  & \tabularnewline


\multicolumn{9}{l}{\textbf{RHR} }\tabularnewline
\qquad{}Supine RHR (bpm)  & 61.48 & 8.68 & 64.46 & 8.28 &  &  &  & \tabularnewline


\multicolumn{9}{l}{\textbf{Cardiorespiratory fitness} }\tabularnewline
\qquad{}VO$_{2}$max per kg BM  & 41.95 & 4.61 & 37.44 & 4.73  & 44.04 & 10.33  & 36.40  & 8.02 \tabularnewline
\qquad{}VO$_{2}$max per kg FFM  & 58.08 & 7.52 & 58.53 & 8.78 &\multicolumn{4}{c}{N.A.}\tabularnewline
\multicolumn{9}{l}{\textbf{Other} }\tabularnewline
\qquad{}\textit{Beta-blocker}  & 22 & 0.42 $\%$ & 15 & 0.26 $\%$ & 67 & 4.62 $\%$ & 58  & 3.64$\%$ \tabularnewline
\bottomrule
\multicolumn{9}{l}{Data are in mean (SD) or n (\%) unless otherwise indicated.}
\tabularnewline


\end{tabular}} 
\end{table}

%Abbreviations: HR: Resting heart rate, bpm: beats per minute, FMI: Fat mass index, PAEE: physical activity energy expenditure, MVPA: Moderate to vigorous physical activity, VPA: Vigorous physical activity

==> table_study_characteristics_short.tex <==
\begin{table*}
%this goes on top
  \caption{\textbf{Characteristics for the study analytical sample: The Fenland I and II studies.} Data is in mean (std). Values with asterisk(*) indicate that this variable comes from Fenland II sensor data which is a smaller cohort (N=2071) due to data filtering (see Figure \ref{fig:flowchart}--Panel 3). The values in FII (future) cohort correspond to the second assessment (7 years later). In Task 1, the training set is FI (present) and the testing set is FII (present) so as to make sure that they come from similar distributions.   %\ds{This table can double as a train/test stats table, since FII is essentially our test set, hence no need for another table}
  } 
\label{tab:cohortcharacteristics}
\resizebox{1\textwidth}{!}{
\begin{tabular}{lllllllllllll}
\toprule
 & \multicolumn{4}{c}{\textbf{Fenland$_{present}$  }} &
 \multicolumn{4}{c}{\textbf{Fenland II$_{future}$ }} &
 \multicolumn{4}{c}{\textbf{Fenland II$_{present}$ }}
 %\tabularnewline
 \\\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
 & \multicolumn{2}{l}{Men (n= 5229)} & \multicolumn{2}{l}{Women (n= 5830)} & \multicolumn{2}{l}{Men (n=1303)} & \multicolumn{2}{l}{Women (n=1372)} & \multicolumn{2}{l}{Men (n=1303)} & \multicolumn{2}{l}{Women (n=1372)}
 %\tabularnewline
 \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
 & \textit{mean}  & \textit{std}  & \textit{mean}  & \textit{std}  & \textit{mean}  & \textit{std}  & \textit{mean}  & \textit{std} & \textit{mean}  & \textit{std} & \textit{mean}  & \textit{std} \tabularnewline
 \midrule
\multicolumn{13}{l}{\textbf{Demographics} }\tabularnewline
\qquad{}Age (years)  & 47.70 & 7.57 & 47.66 & 7.36 & 54.11 & 7.08 & 54.76 & 6.81 & 47.19 & 7.18 & 47.83 & 6.96  \tabularnewline
\multicolumn{13}{l}{\textbf{Anthropometrics} }\tabularnewline
\qquad{}Height (m)  & 1.78 & 0.07 & 1.64 & 0.06 & 1.77 & 0.06 & 1.64 & 0.06 & 1.77 & 0.06 & 1.64 & 0.06\tabularnewline
\qquad{}Body mass (kg)  & 85.85 & 13.83 & 70.54 & 13.92 & 85.31 & 13.59 & 69.58 & 13.77 & 84.85 & 13.14 & 69.04 & 13.26 \tabularnewline
\qquad{}BMI (kg/m$^{2}$)  & 27.16 & 3.97 & 26.17 & 4.97 & 27.03 & 4.01 & 25.85 & 4.94 & 27.00 & 4.03 & 25.84 & 4.98 \tabularnewline

\multicolumn{13}{l}{\textbf{Physical activity} }\tabularnewline
\qquad{}MVPA (min/day)  & 35.87 & 22.35 & 34.40 & 22.59 & 34.92* & 22.18* & 35.35*  & 23.26* & 34.41 & 22.23 & 32.81 & 21.45 \tabularnewline
\qquad{}VPA (min/day)  & 3.27 & 8.57 & 3.31 & 15.67 & 3.57*  & 8.78*  & 3.30*  & 7.52* & 3.38 &9.30 & 3.86 & 27.80 \tabularnewline


\multicolumn{13}{l}{\textbf{Resting Heart Rate} }\tabularnewline
\qquad{}RHR (bpm)  & 61.48 & 8.68 & 64.46 & 8.28 & 59.63*  & 8.28*  & 62.21* & 8.10* & 61.06 & 8.44 & 63.81 & 8.20 \tabularnewline

%we use the REPEATS vo2max here
\multicolumn{13}{l}{\textbf{Cardiorespiratory fitness} }\tabularnewline
\qquad{}VO$_{2}$max (ml $O_2/min/kg$)  & 41.95 & 4.61 & 37.44 & 4.73  & 42.32 & 4.68  & 37.93  & 4.72 & 42.21 & 4.42 & 37.84 & 4.69 \tabularnewline

%\multicolumn{9}{l}{\textbf{Other} }\tabularnewline
%\qquad{}\textit{Beta-blocker}  & 22 & 0.42 $\%$ & 15 & 0.26 $\%$ & 67 & 4.62 $\%$ & 58  & 3.64$\%$ \tabularnewline
\bottomrule
%\multicolumn{9}{l}{Data are in mean (SD) or n (\%) unless otherwise indicated. Values with asterisk(*) indicate that this variable comes from a smaller cohort due to data filtering (see \ref{fig:train_test_llabel} Panel 3).}
\tabularnewline
\end{tabular}
}

\end{table*}

%Abbreviations: HR: Resting heart rate, bpm: beats per minute, FMI: Fat mass index, PAEE: physical activity energy expenditure, MVPA: Moderate to vigorous physical activity, VPA: Vigorous physical activity
